DominoTree: Conditional Tree-Structured Drafting with Domino for Speculative Decoding

Speculative decoding speeds up large language model inference: a small drafter proposes several tokens, and the target model verifies them in one parallel pass. Drafting a tree lets the target verify many alternative continuations at once. DDTree builds such trees from the block-diffusion drafter DFlash, but scores each position independently of the tokens earlier in its branch; Domino conditions on those tokens but drafts only a single chain. DominoTree combines the two: a training-free best-first tree scored by Domino's path-dependent causal correction, restricted to top-M candidates. In a research harness at temperature zero, it averages 5.33x speedup over autoregressive (AR) decoding on Qwen3-4B and 6.89x on Qwen3-8B, peaking at 8.77x; across temperatures it is 20-26% faster than Domino on Qwen3-4B and 27-36% on Qwen3-8B, and 11-20% faster than the stronger of DDTree and its cost-aware variant CaDDTree. A controlled decomposition attributes +10.1% (Qwen3-4B) and +10.7% (Qwen3-8B) accepted length to the correction, and +4.7% and +4.4% to conditioning on the realized path. Served in SGLang on one RTX 5090, it reaches 4.11x and 4.83x AR at batch size 1, 1.17x and 1.09x the speed of Domino's chain, and up to 1.71x AR on 8K-token HELMET summarization, 14-21% above the chain. The lead holds at 2 concurrent requests but reverses from 8 onward, where the chain sustains more goodput despite DominoTree's 28% higher acceptance. DominoTree accepts more tokens than the chain in every serving setting. On the hybrid Gated-DeltaNet Qwen3.6-27B, correct output requires tree-aware recurrent verification; with it, DominoTree matches the chain at batch size 1 (4.58x versus 4.54x AR) and reaches up to 2.11x AR at long context, 15% above the chain.

==> tables/tab-app-helmet-27b.tex <==
\begin{table*}[t]
\centering\footnotesize
\caption{As Table~\ref{tab:app-helmet}, for Qwen3.6-27B (one H200, tree budget 15). \textbf{MTP}
takes EAGLE-3's place, since no EAGLE-3 checkpoint exists for this model.}
\label{tab:app-helmet-27b}
\setlength{\tabcolsep}{3pt}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}ll*{3}{cc}}
\toprule
Task & Method & \multicolumn{2}{c}{8K} & \multicolumn{2}{c}{16K} & \multicolumn{2}{c}{32K} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & & TPS & $\tau$ & TPS & $\tau$ & TPS & $\tau$ \\
\midrule
\multicolumn{8}{c}{\textbf{Qwen3.6-27B}} \\
\midrule
$\infty$Bench-Sum & AR & 64.9 & -- & 60.8 & -- & 53.5 & -- \\
 & MTP & 119.9 & 2.62 & 106.1 & 2.59 & \textbf{84.5} & 2.58 \\
 & DFlash & 107.7 & 2.49 & 95.4 & 2.43 & 78.7 & 2.43 \\
 & Domino & 112.9 & 2.65 & 95.2 & 2.44 & 73.3 & 2.25 \\
 & DominoTree (15) & \textbf{135.9} & \textbf{3.47} & \textbf{113.3} & \textbf{3.24} & 84.0 & \textbf{2.97} \\
 & \quad\emph{vs.\ Domino}, $\Delta$TPS\% & \multicolumn{2}{c}{+20.2 [+18.4,+22.1]} & \multicolumn{2}{c}{+19.0 [+17.6,+20.5]} & \multicolumn{2}{c}{+14.4 [+12.7,+16.2]} \\
 & \quad\emph{vs.\ Domino}, $\Delta\tau$\% & \multicolumn{2}{c}{+31.1 [+29.5,+32.8]} & \multicolumn{2}{c}{+32.5 [+31.0,+34.0]} & \multicolumn{2}{c}{+32.0 [+30.7,+33.4]} \\
\cmidrule(lr){1-8}
Multi-LexSum & AR & 60.1 & -- & 52.0 & -- & 39.4 & -- \\
 & MTP & 112.0 & 2.90 & 87.2 & 2.95 & \textbf{56.8} & 2.98 \\
 & DFlash & 108.7 & 2.98 & 85.0 & 2.98 & 56.6 & 3.01 \\
 & Domino & 117.0 & 3.30 & 86.8 & 3.13 & 55.2 & 2.88 \\
 & DominoTree (15) & \textbf{128.2} & \textbf{4.22} & \textbf{94.0} & \textbf{3.95} & 56.3 & \textbf{3.72} \\
 & \quad\emph{vs.\ Domino}, $\Delta$TPS\% & \multicolumn{2}{c}{+9.6 [+7.8,+11.2]} & \multicolumn{2}{c}{+8.3 [+7.2,+9.5]} & \multicolumn{2}{c}{+2.7 [+0.3,+4.8]} \\
 & \quad\emph{vs.\ Domino}, $\Delta\tau$\% & \multicolumn{2}{c}{+28.0 [+26.4,+29.7]} & \multicolumn{2}{c}{+26.2 [+24.4,+28.1]} & \multicolumn{2}{c}{+29.4 [+27.6,+31.1]} \\
\bottomrule
\end{tabular*}
\end{table*}


==> tables/tab-app-qwen27b-bs1-T00.tex <==
\begin{table*}[t]
\centering\footnotesize
\caption{Qwen3.6-27B bs=1, $T{=}0$, per dataset: one H200 GPU, without tensor parallelism. Speedup over AR and mean accepted length $\tau$; AR runs at 64--68\,tok/s. Per-prompt means merge MT-Bench turns; Overall is the unweighted mean over datasets. There are 50 prompts per dataset (30 for AIME25), with a 2048-token cap. Bold marks the best value per column including ties.}
\label{tab:app-qwen27b-bs1-T00}
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l*{9}{cc}}
\toprule
Method & \multicolumn{6}{c}{Math} & \multicolumn{6}{c}{Code} & \multicolumn{4}{c}{Chat} & \multicolumn{2}{c}{Overall} \\
\cmidrule(lr){2-7}\cmidrule(lr){8-13}\cmidrule(lr){14-17}\cmidrule(lr){18-19}
 & \multicolumn{2}{c}{GSM8K} & \multicolumn{2}{c}{MATH-500} & \multicolumn{2}{c}{AIME25} & \multicolumn{2}{c}{HumanEval} & \multicolumn{2}{c}{MBPP} & \multicolumn{2}{c}{LCB} & \multicolumn{2}{c}{MT-Bench} & \multicolumn{2}{c}{Alpaca} & \multicolumn{2}{c}{Overall} \\
 & Speedup & $\tau$ & Speedup & $\tau$ & Speedup & $\tau$ & Speedup & $\tau$ & Speedup & $\tau$ & Speedup & $\tau$ & Speedup & $\tau$ & Speedup & $\tau$ & Speedup & $\tau$ \\
\midrule
DFlash & 4.71 & 7.42 & 5.33 & 8.05 & 4.65 & 6.84 & 6.24 & 11.02 & \textbf{4.34} & 7.73 & \textbf{3.41} & 5.63 & 3.02 & 4.74 & 2.18 & 3.50 & 4.23 & 6.87 \\
Domino (chain) & \textbf{5.81} & 9.41 & 5.99 & 9.20 & 4.82 & 7.22 & \textbf{6.31} & 11.06 & 4.33 & 7.52 & 3.36 & 5.46 & 3.26 & 5.22 & 2.47 & 3.91 & 4.54 & 7.37 \\
MTP & 2.59 & 3.67 & 2.66 & 3.68 & 2.59 & 3.55 & 2.64 & 3.83 & 2.42 & 3.63 & 2.32 & 3.31 & 2.21 & 3.13 & 2.02 & 2.99 & 2.43 & 3.47 \\
\textbf{DominoTree} & 5.58 & \textbf{9.77} & \textbf{6.06} & \textbf{9.83} & \textbf{5.28} & \textbf{8.36} & 5.80 & \textbf{11.61} & \textbf{4.34} & \textbf{8.07} & 3.30 & \textbf{6.22} & \textbf{3.45} & \textbf{6.02} & \textbf{2.87} & \textbf{4.75} & \textbf{4.58} & \textbf{8.08} \\
\bottomrule
\end{tabular}}
\end{table*}


==> tables/tab-app-qwen27b-bs1-T10.tex <==
\begin{table*}[t]
\centering\footnotesize
\caption{Qwen3.6-27B bs=1, $T{=}1$, per dataset: one H200 GPU, without tensor parallelism. Speedup over AR and mean accepted length $\tau$; AR runs at 65--67\,tok/s. Per-prompt means merge MT-Bench turns; Overall is the unweighted mean over datasets. There are 50 prompts per dataset (30 for AIME25), with a 2048-token cap. Bold marks the best value per column including ties.}
\label{tab:app-qwen27b-bs1-T10}
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l*{9}{cc}}
\toprule
Method & \multicolumn{6}{c}{Math} & \multicolumn{6}{c}{Code} & \multicolumn{4}{c}{Chat} & \multicolumn{2}{c}{Overall} \\
\cmidrule(lr){2-7}\cmidrule(lr){8-13}\cmidrule(lr){14-17}\cmidrule(lr){18-19}
 & \multicolumn{2}{c}{GSM8K} & \multicolumn{2}{c}{MATH-500} & \multicolumn{2}{c}{AIME25} & \multicolumn{2}{c}{HumanEval} & \multicolumn{2}{c}{MBPP} & \multicolumn{2}{c}{LCB} & \multicolumn{2}{c}{MT-Bench} & \multicolumn{2}{c}{Alpaca} & \multicolumn{2}{c}{Overall} \\
 & Speedup & $\tau$ & Speedup & $\tau$ & Speedup & $\tau$ & Speedup & $\tau$ & Speedup & $\tau$ & Speedup & $\tau$ & Speedup & $\tau$ & Speedup & $\tau$ & Speedup & $\tau$ \\
\midrule
DFlash & 4.52 & 7.07 & 5.10 & 7.68 & 4.28 & 6.28 & 6.11 & 10.61 & 4.12 & 7.22 & 3.39 & 5.54 & 2.74 & 4.33 & 1.99 & 3.22 & 4.03 & 6.49 \\
Domino (chain) & 5.50 & 8.74 & 5.50 & 8.39 & 4.50 & 6.67 & \textbf{6.37} & 11.00 & 4.05 & 6.82 & 3.26 & 5.33 & 2.96 & 4.78 & 2.16 & 3.45 & 4.29 & 6.90 \\
MTP & 2.50 & 3.60 & 2.54 & 3.59 & 2.45 & 3.43 & 2.59 & 3.80 & 2.34 & 3.51 & 2.18 & 3.19 & 1.98 & 2.89 & 1.86 & 2.79 & 2.31 & 3.35 \\
\textbf{DominoTree} & \textbf{5.52} & \textbf{9.30} & \textbf{5.59} & \textbf{9.01} & \textbf{4.88} & \textbf{7.69} & 6.22 & \textbf{11.32} & \textbf{4.23} & \textbf{7.63} & \textbf{3.54} & \textbf{6.05} & \textbf{3.24} & \textbf{5.42} & \textbf{2.49} & \textbf{4.24} & \textbf{4.46} & \textbf{7.58} \\
\bottomrule
\end{tabular}}
\end{table*}



==> tables/tab-app-qwen27b-conc.tex <==
\begin{table*}[t]
\centering\footnotesize
\caption{Qwen3.6-27B concurrency, one H200 GPU, without tensor parallelism, $T{=}0$, 512-token generation cap. Columns give goodput (aggregate output tok/s) at each offered concurrency $c$; $\tau$ averages the reported cell means over the sweep; Overall additionally averages datasets. GSM8K/MBPP use 128 prompts; MT-Bench uses 80. Admission caps: DFlash=32, Domino (chain)=32, MTP=32, DominoTree=32, AR=32 (all reach the largest cap probed, 32, on this 141\,GB card). AR is the $\tau{=}1$ reference. Bold marks the best value per column within a dataset.}
\label{tab:app-qwen27b-conc}
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccc}
\toprule
Dataset & Method & $c{=}1$ & $c{=}2$ & $c{=}4$ & $c{=}8$ & $c{=}16$ & $c{=}32$ & $\tau$ \\
\midrule
GSM8K & AR & 67 & 127 & 238 & 426 & 339 & 606 & -- \\
 & DFlash & 309 & 552 & 901 & 1290 & 1171 & 1121 & 7.40 \\
 & Domino (chain) & 384 & 673 & \textbf{1068} & \textbf{1532} & \textbf{1466} & \textbf{1456} & 9.31 \\
 & MTP & 174 & 323 & 572 & 937 & 862 & 1095 & 3.67 \\
 & DominoTree & \textbf{390} & \textbf{674} & 1058 & 1468 & 1373 & 1378 & \textbf{9.77} \\
\midrule
MBPP & AR & 66 & 125 & 227 & 384 & 311 & 514 & -- \\
 & DFlash & 276 & 476 & 744 & 1036 & 1054 & 1050 & 7.66 \\
 & Domino (chain) & 281 & 480 & 757 & \textbf{1083} & \textbf{1078} & \textbf{1091} & 7.51 \\
 & MTP & 163 & 295 & 498 & 774 & 745 & 916 & 3.63 \\
 & DominoTree & \textbf{299} & \textbf{500} & \textbf{775} & 1045 & 1063 & 1060 & \textbf{8.07} \\
\midrule
MT-Bench & AR & 67 & 127 & 236 & 420 & 335 & 583 & -- \\
 & DFlash & 168 & 306 & 515 & 763 & 638 & 638 & 4.86 \\
 & Domino (chain) & 184 & 334 & 559 & 833 & 731 & 727 & 5.41 \\
 & MTP & 146 & 272 & 484 & 794 & 745 & \textbf{926} & 3.16 \\
 & DominoTree & \textbf{221} & \textbf{388} & \textbf{623} & \textbf{890} & \textbf{784} & 767 & \textbf{6.15} \\
\midrule
Overall & AR & 67 & 126 & 234 & 410 & 328 & 568 & -- \\
 & DFlash & 251 & 444 & 720 & 1030 & 954 & 936 & 6.64 \\
 & Domino (chain) & 283 & 496 & 794 & \textbf{1149} & \textbf{1092} & \textbf{1091} & 7.41 \\
 & MTP & 161 & 296 & 518 & 835 & 784 & 979 & 3.49 \\
 & DominoTree & \textbf{304} & \textbf{521} & \textbf{819} & 1134 & 1073 & 1068 & \textbf{8.00} \\
\bottomrule
\end{tabular}}
\end{table*}


==> tables/tab-app-qwen27b-helmet.tex <==
\begin{table*}[t]
\centering\footnotesize
\caption{Qwen3.6-27B HELMET Summarization, one H200 GPU, without tensor parallelism, bs=1, $T{=}0$, 50 prompts/cell, 1200-token generation cap. TPS = total output tokens / total decode time; $\tau$ = mean per-prompt accepted length. \emph{vs.\ Domino} rows give the paired-bootstrap percentage change against the chain [95\% CI], 5000 draws, seed 0, resampling matched prompt indices. The additional \emph{vs.\ MTP} row compares TPS with MTP. CIs compare mean per-prompt TPS, a different estimand from aggregate TPS. $^{*}$ marks a CI containing zero. Bold marks the best TPS and the best $\tau$ per column within a task.}
\label{tab:app-qwen27b-helmet}
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll*{3}{cc}}
\toprule
Task & Method & \multicolumn{2}{c}{8K} & \multicolumn{2}{c}{16K} & \multicolumn{2}{c}{32K} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & & TPS & $\tau$ & TPS & $\tau$ & TPS & $\tau$ \\
$\infty$Bench-Sum & AR & 64.9 & -- & 60.8 & -- & 53.5 & -- \\
 & DFlash & 107.7 & 2.49 & 95.4 & 2.43 & 78.7 & 2.43 \\
 & Domino (chain) & 112.9 & 2.65 & 95.2 & 2.44 & 73.3 & 2.25 \\
 & MTP & 119.9 & 2.62 & 106.1 & 2.59 & \textbf{84.5} & 2.58 \\
 & DominoTree & \textbf{135.9} & \textbf{3.47} & \textbf{113.3} & \textbf{3.24} & 84.0 & \textbf{2.97} \\
 & \quad\emph{vs.\ Domino}, $\Delta$TPS\% & \multicolumn{2}{c}{+20.2 [+18.4,+22.1]} & \multicolumn{2}{c}{+19.0 [+17.6,+20.5]} & \multicolumn{2}{c}{+14.4 [+12.7,+16.2]} \\
 & \quad\emph{vs.\ Domino}, $\Delta\tau$\% & \multicolumn{2}{c}{+31.1 [+29.5,+32.8]} & \multicolumn{2}{c}{+32.5 [+31.0,+34.0]} & \multicolumn{2}{c}{+32.0 [+30.7,+33.4]} \\
 & \quad\emph{vs.\ MTP}, $\Delta$TPS\% & \multicolumn{2}{c}{+13.6 [+11.8,+15.3]} & \multicolumn{2}{c}{+6.7 [+5.7,+7.8]} & \multicolumn{2}{c}{-0.5 [-2.2,+1.4]$^{*}$} \\
\cmidrule(lr){1-8}
Multi-LexSum & AR & 60.1 & -- & 52.0 & -- & 39.4 & -- \\
 & DFlash & 108.7 & 2.98 & 85.0 & 2.98 & 56.6 & 3.01 \\
 & Domino (chain) & 117.0 & 3.30 & 86.8 & 3.13 & 55.2 & 2.88 \\
 & MTP & 112.0 & 2.90 & 87.2 & 2.95 & \textbf{56.8} & 2.98 \\
 & DominoTree & \textbf{128.2} & \textbf{4.22} & \textbf{94.0} & \textbf{3.95} & 56.3 & \textbf{3.72} \\
 & \quad\emph{vs.\ Domino}, $\Delta$TPS\% & \multicolumn{2}{c}{+9.6 [+7.8,+11.2]} & \multicolumn{2}{c}{+8.3 [+7.2,+9.5]} & \multicolumn{2}{c}{+2.7 [+0.3,+4.8]} \\
 & \quad\emph{vs.\ Domino}, $\Delta\tau$\% & \multicolumn{2}{c}{+28.0 [+26.4,+29.7]} & \multicolumn{2}{c}{+26.2 [+24.4,+28.1]} & \multicolumn{2}{c}{+29.4 [+27.6,+31.1]} \\
 & \quad\emph{vs.\ MTP}, $\Delta$TPS\% & \multicolumn{2}{c}{+15.1 [+12.7,+17.2]} & \multicolumn{2}{c}{+8.1 [+6.8,+9.4]} & \multicolumn{2}{c}{-0.1 [-2.6,+2.1]$^{*}$} \\
\bottomrule
\end{tabular}}
\end{table*}


==> tables/tab-qwen27b.tex <==
\begin{table*}[t]
\centering\footnotesize
\caption{Qwen3.6-27B on one H200 GPU (141\,GB), without tensor parallelism, on a different machine from the Qwen3-4B/8B serving experiments. Speedups are normalized to AR within each machine. Batch-size-1 columns average per-dataset speedups and accepted lengths; HELMET speedups average the two task-specific ratios at each length, as in Table~\ref{tab:sglang-longctx}. Goodput is the unweighted mean over GSM8K/MBPP/MT-Bench, as in Table~\ref{tab:sglang-conc}. HELMET $\tau$ averages all six task--length cells; concurrency $\tau$ averages all eighteen dataset--concurrency cells. AR runs at 64--68\,tok/s at batch size 1, 39.4--64.9\,tok/s on HELMET, and 67/568\,tok/s at $c{=}1/32$. DominoTree uses $B{=}15$, $k{=}8$, $M{=}128$ throughout. Bold marks the best printed value per column, including ties.}
\label{tab:qwen27b}
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l*{10}{c}}
\toprule
 & \multicolumn{2}{c}{bs=1, $T{=}0$} & \multicolumn{2}{c}{bs=1, $T{=}1$} & \multicolumn{3}{c}{HELMET} & \multicolumn{3}{c}{Goodput (tok/s)} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
Method & Speedup & $\tau$ & Speedup & $\tau$ & 8K speedup & 32K speedup & $\tau$ & $c{=}1$ & $c{=}32$ & $\tau$ \\
\midrule
DFlash & 4.23 & 6.87 & 4.03 & 6.49 & 1.73 & 1.45 & 2.72 & 251 & 936 & 6.64 \\
Domino (chain) & 4.54 & 7.37 & 4.29 & 6.90 & 1.84 & 1.38 & 2.77 & 283 & \textbf{1091} & 7.41 \\
MTP & 2.43 & 3.47 & 2.31 & 3.35 & 1.85 & \textbf{1.51} & 2.77 & 161 & 979 & 3.49 \\
DominoTree & \textbf{4.58} & \textbf{8.08} & \textbf{4.46} & \textbf{7.58} & \textbf{2.11} & 1.50 & \textbf{3.60} & \textbf{304} & 1068 & \textbf{8.00} \\
\bottomrule
\end{tabular}}
\end{table*}


